CHANG-ES XVI: An in-depth view of the cosmic-ray transport in the edge-on spiral galaxies NGC 891 and NGC 4565

Cosmic-ray electrons (CREs) originating from the star-forming discs of spiral galaxies frequently form extended radio haloes that are best observable in edge-on galaxies. For the present study we selected two nearby edge-on galaxies from the CHANG-ES survey, NGC 891 and 4565, which differ largely in halo size and SFR. To figure out how such differences are related to the CRE transport in disc and halo, we use wide-band 1.5 and 6 GHz VLA observations obtained in the B, C, and D configurations, and combine the 6 GHz images with Effelsberg observations to correct for missing short spacings. We study the spatially resolved non-thermal spectral index distribution in terms of CRE spectral ageing, compute total magnetic field strengths assuming energy equipartition between CRs and magnetic fields, and also determine synchrotron scale heights. Based on the vertical profiles of synchrotron intensity and spectral index, we create purely advective and purely diffusive CRE transport models by numerically solving the 1D diffusion-loss equation. In particular, we investigate for the first time the radial dependence of synchrotron and magnetic field scale heights, advection speeds and diffusion coefficients in these two galaxies. We find the spectral index distribution of NGC 891 to be mostly consistent with continuous CRE injection, while in NGC 4565 the local synchrotron spectra are more in line with discrete-epoch CRE injection (JP or KP models). This implies that CRE injection timescales are lower than the synchrotron cooling timescales. The scale height of NGC 891 increases with radius, indicating that synchrotron losses are significant. NGC 891 is probably dominated by advective CRE transport at a velocity of $\gtrsim150\,\mathrm{km\,s^{-1}}$. In contrast, NGC 4565 is diffusion-dominated up to $z=1$ kpc or higher, with a diffusion coefficient of $\geq2\times10^{28}\,\mathrm{cm^2\,s^{-1}}$.

==> fltpoint.tex <==
%%
%% This is file `fltpoint.tex',
%% generated with the docstrip utility.
%%
%% The original source files were:
%%
%% fltpoint.dtx  (with options: `fltmain')
%% 
%% IMPORTANT NOTICE:
%% 
%% For the copyright see the source file.
%% 
%% Any modified versions of this file must be renamed
%% with new filenames distinct from fltpoint.tex.
%% 
%% For distribution of the original source see the terms
%% for copying and modification in the file fltpoint.dtx.
%% 
%% This generated file may be distributed as long as the
%% original source files, as listed above, are part of the
%% same distribution. (The sources need not necessarily be
%% in the same archive or directory.)
\edef\atcatcode{\the\catcode`\@}
\catcode`\@=11
\ifx\documentclass\relax
\long\def\@ifnextchar#1#2#3{%
  \let\reserved@d=#1%
  \def\reserved@a{#2}%
  \def\reserved@b{#3}%
  \futurelet\@let@token\@ifnch}
\def\@ifnch{%
  \ifx\@let@token\@sptoken
    \let\reserved@c\@xifnch
  \else
    \ifx\@let@token\reserved@d
      \let\reserved@c\reserved@a
    \else
      \let\reserved@c\reserved@b
    \fi
  \fi
  \reserved@c}
\def\:{\let\@sptoken= } \:
\def\:{\@xifnch} \expandafter\def\: {\futurelet\@let@token\@ifnch}
\fi
\def\iloop#1\irepeat{\def\ibody{#1}\iiterate}
\def\iiterate{\ibody\let\inext=\iiterate\else\let\inext=\relax\fi
   \inext}
\def\xloop#1\xrepeat{\def\xbody{#1}\xiterate}
\def\xiterate{\xbody\let\xnext\xiterate\else\let\xnext\relax\fi\xnext}
\let\repeat\fi
\let\irepeat\fi
\let\xrepeat\fi
\newcount\fp@loopcount
\newcount\fp@loopcountii
\newcount\fp@result
\newcount\fp@carryover
\newcount\fp@tempcount
\newcount\fp@tempcountii
\def\fp@setparam#1{\xdef\fp@param{#1}}%
\def\ar@set#1#2#3{\expandafter\edef\csname#1@\number#2\endcsname{%
   \number#3}}
\def\ar@get#1#2{\csname#1@\number#2\endcsname}
\def\ar@setsig#1#2{\expandafter\edef\csname#1@sig\endcsname{#2}}
\def\ar@getsig#1{\csname#1@sig\endcsname}
\def\ar@getul#1{\csname#1@ul\endcsname}
\def\ar@getll#1{\csname#1@ll\endcsname}
\def\ar@setul#1#2{\expandafter\edef\csname#1@ul\endcsname{\number#2}}
\def\ar@setll#1#2{\expandafter\edef\csname#1@ll\endcsname{\number#2}}
\def\fp@settomax#1#2#3{%
   \ifnum#2<#3\relax
      #1=#3\relax
   \else
      #1=#2\relax
   \fi
}
\def\fp@settomin#1#2#3{%
   \ifnum#2<#3\relax
      #1=#2\relax
   \else
      #1=#3\relax
   \fi
}
\def\fp@modulo#1#2{%
   \fp@tempcount=#1\relax
   \fp@tempcountii=#1\relax
   \divide\fp@tempcountii#2\relax
   \multiply\fp@tempcountii#2\relax
   \advance\fp@tempcount-\fp@tempcountii
   \edef\fp@param{\number\fp@tempcount}}
\def\fp@regread#1#2{%
   \fp@regread@raw{#1}{#2}%
   \fp@cleanreg{#1}}
\def\fp@regread@raw#1#2{%
   \fp@tempcount=0
   \edef\fp@arrayname{#1}%
   \ar@setsig{#1}{+}%
   \edef\fp@scratch{#2\fp@decimalsign}%
   \expandafter\fp@readchars\fp@scratch\end
   \ifnum\ar@getul{#1}=-1
      \ar@setul{#1}{0}%
      \ar@set{#1}{0}{0}%
   \fi
   \fp@tempcount=0
   \fp@tempcountii=\ar@getul{#1}\relax
   \iloop
   \ifnum\fp@tempcount<\fp@tempcountii
      \edef\fp@scratch{\ar@get{#1}{\fp@tempcountii}}%
      \ar@set{#1}{\fp@tempcountii}{\ar@get{#1}{\fp@tempcount}}%
      \ar@set{#1}{\fp@tempcount}{\fp@scratch}%
      \advance\fp@tempcount by 1
      \advance\fp@tempcountii by -1
   \irepeat
}% end \fp@regread@raw
\def\fp@readchars#1{%
   \ifx#1\end
      \let\inext=\relax
      \ifnum\fp@tempcount<0
         \advance\fp@tempcount by 1
         \ar@setll{\fp@arrayname}{\fp@tempcount}%
      \else
         \ar@setll{\fp@arrayname}{0}%
      \fi
   \else % \ifx#1\end
      \let\inext=\fp@readchars
      \ifx#1+%
      \else
         \ifx#1-%
            \if\ar@getsig{\fp@arrayname}-%
               \ar@setsig{\fp@arrayname}{+}%
            \else
               \ar@setsig{\fp@arrayname}{-}%
            \fi
         \else
            \if\noexpand#1\fp@decimalsign%
               \ifnum\fp@tempcount>-1
                  \advance\fp@tempcount by -1
                  \ar@setul{\fp@arrayname}{\fp@tempcount}%
                  \fp@tempcount=-1
               \fi
            \else
               \ar@set{\fp@arrayname}{\fp@tempcount}{#1}%
               \ifnum\fp@tempcount<0
                  \advance\fp@tempcount by -1
               \else
                  \advance\fp@tempcount by 1
               \fi
            \fi% end \if\noexpand#1\fp@decimalsign
         \fi% end \ifx#1-
      \fi% end \ifx#1+
   \fi% end \ifx#1\end
   \inext
}% end \fp@readchars
\def\fp@regget#1#2{%
   \if\ar@getsig{#1}-%
      \def#2{-}%
   \else
      \def#2{}%
   \fi
   \fp@tempcount=\ar@getul{#1}\relax
   \iloop
      \ifnum\fp@tempcount=-1
         \edef#2{#2\fp@decimalsign}%
      \fi
      \edef#2{#2\ar@get{#1}{\fp@tempcount}}%
   \ifnum\fp@tempcount>\ar@getll{#1}\relax
      \advance\fp@tempcount by -1
   \irepeat
}% end \def\fp@regget
\def\fp@cleanreg#1{%
   \fp@tempcount=\ar@getul{#1}\relax
   \iloop
   \ifnum\fp@tempcount>0
      \ifnum\ar@get{#1}{\fp@tempcount}=0
         \advance\fp@tempcount by -1
         \ar@setul{#1}{\fp@tempcount}%
      \else
         \fp@tempcount=0
      \fi
   \irepeat
   \fp@tempcount=\ar@getll{#1}\relax
   \iloop
   \ifnum\fp@tempcount<0
      \ifnum\ar@get{#1}{\fp@tempcount}=0
         \advance\fp@tempcount by 1
         \ar@setll{#1}{\fp@tempcount}%
      \else
         \fp@tempcount=0
      \fi
   \irepeat
   \ifnum\ar@getll{#1}=\ar@getul{#1}\relax
      \ifnum\ar@get{#1}{0}=0\relax
         \ar@setsig{#1}{+}%
      \fi
   \fi
}% end \fp@regclean
\def\fp@getdigit#1#2{%
   \ifnum#2<\ar@getll{#1}\relax
      \fp@setparam0%
   \else
      \ifnum#2>\ar@getul{#1}\relax
         \fp@setparam0%
      \else
         \fp@setparam{\ar@get{#1}{#2}}%
      \fi
   \fi
}% end \fp@getdigit
\def\fp@shiftright#1#2{%
   \edef\fp@shiftamount{\number#2}%
   \fp@settomax{\fp@tempcount}{\ar@getul{#1}}{-\fp@shiftamount}%
   \fp@settomin{\fp@tempcountii}{\ar@getll{#1}}{-\fp@shiftamount}%
   \def\fp@shiftnum{}%
   \iloop
      \fp@getdigit{#1}{\fp@tempcount}%
      \edef\fp@shiftnum{\fp@shiftnum\fp@param}%
      \ifnum\fp@tempcount=-\fp@shiftamount\relax
         \edef\fp@shiftnum{\fp@shiftnum\fp@decimalsign}%
      \fi
   \ifnum\fp@tempcount>\fp@tempcountii
      \advance\fp@tempcount by -1
   \irepeat
   \fp@regread{#1}{\fp@shiftnum}%
}% end \fp@shiftright
\def\fp@firstnonzero#1{%
   \fp@regcomp{#1}{@0}%
   \if\fp@param=%
      \fp@setparam0%
   \else
      \fp@tempcount=\ar@getul{#1}\relax%
      \fp@tempcountii=\ar@getll{#1}\relax%
      \iloop
         \ifnum\ar@get{#1}{\fp@tempcount}>0
            \fp@setparam{\number\fp@tempcount}%
            \fp@tempcount=\fp@tempcountii
         \fi
      \ifnum\fp@tempcount>\fp@tempcountii
         \advance\fp@tempcount by -1
      \irepeat
   \fi
}% end \fp@firstnonzero
\def\fp@regcomp#1#2{%
   {%
      \if\ar@getsig{#1}-%
         \if\ar@getsig{#2}-%
            \fp@regcomp@main{#1}{#2}<>%
         \else
            \fp@setparam{<}%
         \fi
      \else
         \if\ar@getsig{#2}-%
            \fp@setparam{>}%
         \else
            \fp@regcomp@main{#1}{#2}><%
         \fi
      \fi
   }%
}
\def\fp@regcomp@main#1#2#3#4{%
   \fp@settomax{\fp@loopcount}{\ar@getul{#1}}{\ar@getul{#2}}%
   \fp@settomin{\fp@loopcountii}{\ar@getll{#1}}{\ar@getll{#2}}%
   \loop
      \fp@getdigit{#1}{\fp@loopcount}%
      \fp@tempcount=\fp@param\relax
      \fp@getdigit{#2}{\fp@loopcount}%
      \fp@tempcountii=\fp@param\relax
      \ifnum\fp@tempcount<\fp@tempcountii
         \fp@setparam{#4}%
         \fp@loopcount=\fp@loopcountii
      \else
         \ifnum\fp@tempcount>\fp@tempcountii
            \fp@setparam{#3}%
            \fp@loopcount=\fp@loopcountii
         \else
            \ifnum\fp@loopcount=\fp@loopcountii
               \fp@setparam{=}%
            \fi
         \fi
      \fi
   \ifnum\fp@loopcount>\fp@loopcountii
      \advance\fp@loopcount by -1
   \repeat
}% end \fp@regcomp@main
\def\fp@regabs#1{%
   \ar@setsig{#1}{+}%
}
\def\fp@regneg#1{%
   \if\ar@getsig{#1}-%
      \ar@setsig{#1}{+}%
   \else
      \fp@regcomp{#1}{@0}%
      \if\fp@param=%
      \else
         \ar@setsig{#1}{-}%
      \fi
   \fi
}
\def\fp@reground#1#2{%
   \ifnum#2>\ar@getll{#1}\relax
      {%
         \fp@tempcount=#2\relax
         \advance\fp@tempcount by -1
         \fp@getdigit{#1}{\fp@tempcount}%
         \ifnum\fp@param>4
            \fp@regcopy{fp@temp}{@1}%
            \fp@shiftright{fp@temp}{#2}%
            \fp@regcomp{#1}{@0}%
            \if\fp@param<%
               \fp@regneg{fp@temp}%
            \fi
            \fp@regadd{#1}{fp@temp}%
         \fi
         \ifnum#2>0
            \fp@loopcount=#2\relax
            \iloop
               \ifnum\fp@loopcount>0
                  \advance\fp@loopcount by -1
                  \ar@set{#1}{\fp@loopcount}{0}%
            \irepeat
            \ar@setll{#1}{0}%
         \else
            \ar@setll{#1}{#2}%
         \fi
         \fp@regget{#1}{\fp@scratch}%
         \fp@setparam\fp@scratch
      }%
      \fp@regread{#1}{\fp@param}%
   \fi
} % end \fp@reground
\def\fp@regcopy#1#2{%
   \fp@regget{#2}{\fp@scratch}%
   \fp@regread{#1}{\fp@scratch}%
}
\def\fp@regadd#1#2{%
   {%
      \if\ar@getsig{#1}\ar@getsig{#2}%
         \fp@settomin{\fp@loopcount}{\ar@getll{#1}}{\ar@getll{#2}}%
         \edef\fp@add@start{\number\fp@loopcount}%
         \fp@settomax{\fp@tempcount}{\ar@getul{#1}}{\ar@getul{#2}}%
         \edef\fp@add@finish{\number\fp@tempcount}%
         \fp@carryover=0
         \loop
            \fp@getdigit{#1}{\fp@loopcount}%
            \fp@result=\fp@param\relax
            \fp@getdigit{#2}{\fp@loopcount}%
            \advance\fp@result by \fp@param\relax
            \advance\fp@result by \fp@carryover
            \ifnum\fp@result>9
               \fp@carryover=1
               \advance\fp@result by -10
            \else
               \fp@carryover=0
            \fi
            \ar@set{#1}{\fp@loopcount}{\fp@result}%
         \ifnum\fp@loopcount<\fp@add@finish\relax
            \advance\fp@loopcount by 1
         \repeat
         \ifnum\fp@carryover>0
            \advance\fp@loopcount by 1
            \ar@set{#1}{\fp@loopcount}{\fp@carryover}%
         \fi
         \ar@setll{#1}{\fp@add@start}%
         \ar@setul{#1}{\fp@loopcount}%
         \fp@regget{#1}{\fp@scratch}%
         \fp@setparam\fp@scratch
      \else % \if sign
         \fp@regcopy{fp@tempi}{#1}%
         \fp@regcopy{fp@tempii}{#2}%
         \fp@regabs{fp@tempi}%
         \fp@regabs{fp@tempii}%
         \fp@regcomp{fp@tempi}{fp@tempii}%
         \if\fp@param>%
            \fp@regadd@sub{#1}{fp@tempi}{fp@tempii}%
         \else
            \fp@regadd@sub{#2}{fp@tempii}{fp@tempi}%
         \fi
      \fi % end \if sign
   }%
   \fp@regread{#1}{\fp@param}%
}% end \fp@regadd
\def\fp@regadd@sub#1#2#3{%
   \fp@regsub@restricted{#2}{#3}%
   \fp@regcomp{#1}{@0}%
   \if\fp@param<%
      \fp@regneg{#2}%
   \fi
   \fp@regget{#2}{\fp@scratch}%
   \fp@setparam\fp@scratch
}% end \fp@regadd@sub
\def\fp@regsub@restricted#1#2{%
   {%
      \fp@settomin{\fp@loopcount}{\ar@getll{#1}}{\ar@getll{#2}}%
      \edef\fp@lowermin{\number\fp@loopcount}%
      \fp@settomax{\fp@tempcount}{\ar@getul{#1}}{\ar@getul{#2}}%
      \edef\fp@uppermin{\number\fp@tempcount}%
      \fp@carryover=0
      \loop
         \fp@getdigit{#1}{\fp@loopcount}%
         \fp@result=\fp@param\relax
         \fp@getdigit{#2}{\fp@loopcount}%
         \advance\fp@result by -\fp@param\relax
         \advance\fp@result by \fp@carryover
         \ifnum\fp@result<0
            \fp@carryover=-1
            \advance\fp@result by 10
         \else
            \fp@carryover=0
         \fi
         \ar@set{#1}{\fp@loopcount}{\fp@result}%
      \ifnum\fp@loopcount<\fp@uppermin\relax
         \advance\fp@loopcount by 1
      \repeat
      \ifnum\fp@carryover=-1
         \advance\fp@loopcount by 1
         \ar@set{#1}{\fp@loopcount}{-1}%
      \fi
      \ar@setll{#1}{\fp@lowermin}%
      \ar@setul{#1}{\fp@loopcount}%
   \fp@regget{#1}{\fp@scratch}%
   \fp@setparam\fp@scratch
   }%
   \fp@regread{#1}{\fp@param}%
}% end \fp@regsub@restricted
\def\fp@regsub#1#2{%
   {%
      \fp@regneg{#2}%
      \fp@regadd{#1}{#2}%
      \fp@regget{#1}{\fp@scratch}%
      \fp@setparam\fp@scratch
   }%
   \fp@regread{#1}{\fp@param}%
}
\def\fp@regmul#1#2{%
   {%
      \fp@regcopy{fp@temp1}{@0}%
      \fp@loopcountii=\ar@getll{#2}\relax
      \xloop
         \fp@loopcount=\ar@getll{#1}\relax
         \fp@carryover=0
         \def\fp@newnum{}%
         \loop
            \fp@result=\ar@get{#2}{\fp@loopcountii}\relax
            \multiply\fp@result by \ar@get{#1}{\fp@loopcount}\relax
            \advance\fp@result by \fp@carryover
            \ifnum\fp@result>9
               \fp@carryover=\fp@result
               \divide\fp@carryover by 10
               \fp@tempcount=\fp@carryover
               \multiply\fp@tempcount by 10
               \advance\fp@result by -\fp@tempcount
            \else
               \fp@carryover=0
            \fi
            \edef\fp@newnum{\number\fp@result\fp@newnum}%
         \ifnum\fp@loopcount<\ar@getul{#1}\relax
            \advance\fp@loopcount by 1
         \repeat
         \edef\fp@newnum{\number\fp@carryover\fp@newnum}%
         \fp@regread{fp@temp2}{\fp@newnum}%
         \fp@tempcount=\fp@loopcountii
         \advance\fp@tempcount by -\number\ar@getll{#2}\relax
         \fp@shiftright{fp@temp2}{\fp@tempcount}%
         \fp@regadd{fp@temp1}{fp@temp2}%
      \ifnum\fp@loopcountii<\ar@getul{#2}\relax
         \advance\fp@loopcountii by 1
      \xrepeat
      \fp@tempcount=\ar@getll{#1}\relax
      \advance\fp@tempcount by \ar@getll{#2}\relax
      \fp@shiftright{fp@temp1}{\fp@tempcount}%
      \if\ar@getsig{#1}\ar@getsig{#2}%
      \else
         \fp@regneg{fp@temp1}%
      \fi
   \fp@regget{fp@temp1}{\fp@scratch}%
   \fp@setparam\fp@scratch
   }%
   \fp@regread{#1}{\fp@param}%
} % end \fp@regmul
\def\fp@regdiv#1#2{%
   {%
      \fp@regcopy{fp@temp1}{#1}%
      \fp@regcopy{fp@temp2}{#2}%
      \fp@regabs{fp@temp1}%
      \fp@regabs{fp@temp2}%
      \fp@firstnonzero{fp@temp1}%
      \fp@loopcountii=\fp@param\relax
      \fp@firstnonzero{fp@temp2}%
      \advance\fp@loopcountii by -\fp@param\relax
      \fp@shiftright{fp@temp2}{\fp@loopcountii}%
      \def\fp@divnum{}%
      \ifnum\fp@loopcountii<0
         \fp@tempcount=\fp@loopcountii
         \loop
         \ifnum\fp@tempcount<-1
            \edef\fp@divnum{0\fp@divnum}%
            \advance\fp@tempcount by 1
         \repeat
         \edef\fp@divnum{\fp@decimalsign\fp@divnum}%
      \fi
      \xloop
      \fp@tempcount=\fp@loopcountii
      \advance\fp@tempcount by 1
      \ifnum\fp@tempcount>-\fp@accuracy\relax
         \fp@loopcount=0
         \loop
            \fp@regcomp{fp@temp2}{fp@temp1}%
            \if\fp@param=%
               \def\fp@accuracy{0}%
               \gdef\fp@param{<}%
            \fi
         \if\fp@param<%
            \fp@regsub@restricted{fp@temp1}{fp@temp2}%
            \advance\fp@loopcount by 1
         \repeat
         \ifnum\fp@loopcountii=-1
            \edef\fp@divnum{\fp@divnum\fp@decimalsign}%
         \fi
         \edef\fp@divnum{\fp@divnum\number\fp@loopcount}%
         \fp@shiftright{fp@temp2}{-1}%
         \advance\fp@loopcountii by -1
      \xrepeat
      \if\ar@getsig{#1}\ar@getsig{#2}%
         \fp@regread{fp@temp1}{\fp@divnum}%
      \else
         \fp@regread{fp@temp1}{-\fp@divnum}%
      \fi
      \fp@regget{fp@temp1}{\fp@scratch}%
      \fp@setparam\fp@scratch
   }%
   \fp@regread{#1}{\fp@param}%
}
\def\fp@call@bin#1#2#3#4{%
   {%
      \fp@regread{fp@user1}{#2}%
      \fp@regread{fp@user2}{#3}%
      \csname fp@reg#4\endcsname{fp@user1}{fp@user2}%
      \fp@regget{fp@user1}{\fp@scratch}%
      \fp@setparam\fp@scratch
   }%
   \edef#1{\fp@param}%
}
\def\fpAdd#1#2#3{\fp@call@bin{#1}{#2}{#3}{add}}
\def\fpSub#1#2#3{\fp@call@bin{#1}{#2}{#3}{sub}}
\def\fpMul#1#2#3{\fp@call@bin{#1}{#2}{#3}{mul}}
\def\fpDiv#1#2#3{\fp@call@bin{#1}{#2}{#3}{div}}
\def\fp@call@un#1#2#3{%
   {%
      \fp@regread{fp@user1}{#2}%
      \csname fp@reg#3\endcsname{fp@user1}%
      \fp@regget{fp@user1}{\fp@scratch}%
      \fp@setparam\fp@scratch
   }%
   \edef#1{\fp@param}%
}
\def\fpAbs#1#2{\fp@call@un{#1}{#2}{abs}}
\def\fpNeg#1#2{\fp@call@un{#1}{#2}{neg}}
\def\fpRound#1#2#3{%
   {%
      \fpRegSet{fp@user1}{#2}%
      \fpRegRound{fp@user1}{#3}%
      \fpRegGet{fp@user1}{\fp@scratch}%
      \fp@setparam\fp@scratch
   }%
   \edef#1{\fp@param}%
}
\def\fpRegSet#1#2{\fp@regread{#1}{#2}}
\def\fpRegGet#1#2{\fp@regget{#1}{#2}}
\def\fpRegAdd#1#2{\fp@regadd{#1}{#2}}
\def\fpRegSub#1#2{\fp@regsub{#1}{#2}}
\def\fpRegMul#1#2{\fp@regmul{#1}{#2}}
\def\fpRegDiv#1#2{\fp@regdiv{#1}{#2}}
\def\fpRegAbs#1{\fp@regabs{#1}}
\def\fpRegNeg#1{\fp@regneg{#1}}
\def\fpRegCopy#1#2{\fp@regcopy{#1}{#2}}
\def\fpRegRound#1#2{\fp@reground{#1}{#2}}
\def\fpAccuracy#1{\edef\fp@accuracy{#1}}
\fpAccuracy{5}
\def\fpDecimalSign#1{\edef\fp@decimalsign{#1}}
\fpDecimalSign{,}
\def\fpThousandSep#1{\edef\fp@thousandsep{#1}}
\fpThousandSep{}
\fp@regread{@0}{0}
\fp@regread{@1}{1}
\catcode`\@=\atcatcode\relax
\endinput
%%
%% End of file `fltpoint.tex'.

